A Graph-based Model for GPU Caching Problems

Modeling data sharing in GPU programs is a challenging task because of the massive parallelism and complex data sharing patterns provided by GPU architectures. Better GPU caching efficiency can be achieved through careful task scheduling among different threads. Traditionally, in the field of parallel computing, graph partition models are used to model data communication and guide task scheduling. However, we discover that the previous methods are either inaccurate or expensive when applied to GPU programs. In this paper, we propose a novel task partition model that is accurate and gives rise to the development of fast and high quality task/data reorganization algorithms. We demonstrate the effectiveness of the proposed model by rigorous theoretical analysis of the algorithm bounds and extensive experimental analysis. The experimental results show that it achieves significant performance improvement across a representative set of GPU applications.

==> abstract.tex <==
%The massive amount of fine-grained parallelism exposed by a GPU program makes it difficult to
%exploit shared cache benefits even there is good program locality. The non deterministic feature of
%thread execution in the bulk synchronize parallel (BSP) model makes the situation even worse.

%Most prior work in exploiting GPU cache sharing focuses on regular applications that have linear
%memory access indices. In this paper, we formulate a generic workload partitioning model that
%systematically exploits the complexity and approximation bound for optimal cache sharing among GPU
%threads. Our exploration in this paper demonstrates that it is possible to utilize GPU cache
%efficiently without significant programming overhead or ad-hoc application-specific
%implementation.

%The massive amount of fine-grained parallelism exposed by
%a GPU program makes it difficult to exploit shared cache
%benefits even there is good program locality.
%Most prior work on GPU memory performance focuses
%on regular applications that have linear memory access indices or regular applications whose memory accesses are not coalesced. None of prior work systematically explore data reuse in GPU programs.
%In this paper, we propose a simple yet effective locality model that allows for bounding analysis and give rise to effective. polynomial algorithms. Our techniques improve GPU performance by up to 2.1 times and has almost no slow down when there is little data reuse.

Modeling data sharing in GPU programs is a challenging task because of the massive parallelism and complex data sharing patterns provided by GPU architectures.
Better GPU caching efficiency can be achieved through careful task scheduling among different threads.
Traditionally, in the field of parallel computing, graph partition models are used to model data communication and guide task scheduling. However, we discover that the previous methods are either inaccurate or expensive when applied to GPU programs.
%More specifically, these models are usually task-centric and do not describe data communication accurately. And the overhead is intolerable when the number of parallel tasks is large.
In this paper, we propose a novel task partition model that is accurate and gives rise to the development of fast and high quality task/data reorganization algorithms.
We demonstrate the effectiveness of the proposed model by rigorous theoretical analysis of the algorithm bounds and extensive experimental analysis.
The experimental results show that it achieves significant performance improvement across a representative set of GPU applications.



==> append.tex <==
\newpage
\subsection*{Appendix}

\subsubsection*{NP-completeness of the balanced edge partition problem}
It is easy to prove,  by a reduction from the NP-hard {\sf \bf partition problem},  %add citation
%later
that the {\em k-way} balanced edge partition problem is NP-hard, even for $k=2$. 

We briefly sketch the reduction. Recall that in the 
partition problem we are given a
set $S$ of positive integers $a_1,a_2,...,a_n$, and our task is to decide if the numbers can be
partitioned into two subsets $S_1$ and $S_2$ such that the sum of numbers in $S_1$ equals the sum of
the numbers in $S_2$. 

In the reduction we construct a graph with $n$ {\em cycles} $c_1,c_2,...,c_n$ such that
$|C_i|=a_i$. Obviously, a  partition $(S_{1},S_{2})$ for the instance  of the partition problem exists if and only if the
2$-$way balanced edge partition problem reduce from it has a minimal communication cost of 1. 


\subsubsection*{The case that a real/original edge is cut}
\medskip

\noindent {\bf \sf \underline{Edge Fixing}} 

\medskip

If the cut set of $D'$ contains a real edge, one end point of the this edge needs to be moved
to the cluster of the other end point.

Since the above manipulation will upset equality between clusters, in order to minimize (and eventually eliminate) the harm
caused by the moves,
we process real edges that cross between different clusters in the following order.

We cycle through all pairs $(A', B')$ of clusters and do as follows:
For the current pair $(A', B')$ of clusters we first find the set $R_{A',B'}$ of real edges that cross
between $A'$ and $B'$. Then we put half of the edges of $R_{A',B'}$ entirely into $A'$
and the other half entirely into $B'$. If $|R_{A',B'}|$ is odd, we choose a single edge from it and leave 
its end points in the same clusters as they were originally (i.e. in $A'$ and $B'$).
It is easy to see that restructuring the clusters as above leaves them balanced.

Consider now every cluster as a ``super-node,'' and form an edge
between two super-nodes if after the restructuring there is an edge between the corresponding clusters.
A graph will arises on the super-nodes that we call $C'$. 

For technical reasons we shall assume that the cluster size, $2m/k$, is even (this is a natural assumption, since if $k$ does not divide $m$,
the original problem cannot be solved). 
We argue that in this case the
degree of every super-node in $C'$ is even: Take out the inner-cluster edges together with their
end-points in $D'$., and all we are left with are nodes of internal real edges (that are not
cut), with an even number of end points. Thus the number of edges going out of a cluster must be even too.     

Since $C'$ has only even degree vertices, its edge set decomposes into Euler-tours that can be made directed in an obvious way. 
In a final stage we can fix edges along these directed Euler tours by 
restructuring the clusters once more, at this time putting each inter-cluster edge into the cluster associated with its starting point in the directed Euler tour.
It is easy to see that after this final restructuring of clusters they remain of equal size.

Edge-fixing process can be designed in a more sophisticated way rather than arbitrarily picking
pairs of clusters and cut real edges, which we will describe in Section \ref{sec:psf}. 



==> conclusion.tex <==
\section{Conclusion}

We formulate a generic graph partitioning model that systematically exploits the
complexity and analytical bound for the optimal cache data reuse problem in GPU
computing.
Our experiments show that our method can improve data sharing and performance significantly for GPU benchmarks.
Our exploration in this paper demonstrates for the first time that it is feasible to use graph
partitioning models to enhance GPU cache performance.


==> eval.tex <==
\section{Evaluation}
\label{sec:eval}

\subsection{Experiment Setup}

Our hardware platform is a machine with NVIDIA GeForce GTX680 GPU. The GTX680
has CUDA computing capability 3.0. It has 8 streaming multiprocessors (SM) with
192 cores on each of them. On each SM there is 64 KB of L1 cache and shared
memory in total, shared by 192 cores. There are three size configurations of L1
cache and shared memory: 16KB/48KB, 32KB/32KB and 48KB/16KB. Since L1 cache in
GTX680 is allowed for local memory data only, we always configure L1 cache to be
16KB. There is also 48KB read-only (texture) cache. The CPU is Intel Core
i7-4790 at 3.6 GHz with 8MB cache.  

We use seven representative applications including Rodinia benchmark suite
\cite{Che+:IISWC09} and the CUSP\cite{CUSP} library. The benchmarks are listed in Table
\ref{tbl:bench}. In these seven benchmarks, the \emph{CG} benchmark calls sparse matrix vector
multiplication kernel
extensively and we perform optimization on sparse matrix vector multiplication
kernel. We also compare our sparse matrix vector multiplication kernel
performance with that of CUSPARSE, which is a highly optimized and well adopted
GPU sparse linear algebra library \cite{CUSPARSE}. 

We use the input sets coming with the benchmark suite or real-world input sets.
For example, the \emph{Cfd} benchmark from Rodinia benchmark suite \cite{Che+:IISWC09}
has three input meshes. For sparse matrix input to \emph{Cg}, we matrices from the University of Florida sparse matrix collection
\cite{FloridaMat} and matrix market \cite{MATRIXMARKET}. All programs are
compiled on a system that runs 64-bit Linux with kernel version 3.1.10 and CUDA 5.5. 

\citexx
\begin{table}[t]
\centering
\footnotesize
\caption{Benchmarks}
%\scriptsize
%\begin{tabularx}{0.85\linewidth}{Xcccccc}
\begin{tabular}{|l|l|l} \hline
Benchmark & Description & Input\\
\hline
b+tree \cite{Che+:IISWC09} & Tree data structure. & Queries to database of 1
million records.   \\
bfs \cite{Che+:IISWC09}  & Breadth first search  & \\
cfd \cite{Che+:IISWC09}  & Comp. fluid dynamics  & 97K, 193K, 0.2M node meshes. \\
gaussian \cite{Che+:IISWC09}  & Gaussian elimination  \\
particlefilter \cite{Che+:IISWC09}  & SMC for posterio density estimation  \\
streamcluster \cite{Che+:IISWC09}  & Data stream clustering    \\
spmv \cite{CUSP} & Sparse matrix multiplication \\
\hline
\end{tabular}
\label{tbl:bench}
\end{table}



%For every benchmark, we run five times to get an average of running time. We also vary the thread
%block sizes to see the impact of data sharing at different work cluster sizes. 

\begin{figure*}
\centering
%\begin{subfigure}[b]{0.3\textwidth}
%\centering
\subfloat[B+tree]{\includegraphics[width=0.3\textwidth]{figures/B+tree.pdf}}
\subfloat[Bfs]{\includegraphics[width=0.3\textwidth]{figures/BFS.pdf}}
\subfloat[CFD]{\includegraphics[width=0.3\textwidth]{figures/CFD.pdf}} \hfill
\subfloat[Gaussian]{\includegraphics[width=0.3\textwidth]{figures/Gaussian.pdf}}
\subfloat[Particle
filter]{\includegraphics[width=0.3\textwidth]{figures/particleFilter.pdf}}
\subfloat[Streamcluster]{\includegraphics[width=0.3\textwidth]{figures/streamcluster.pdf}}
\caption{Application performance on different block sizes}
\label{fig:appspec}
\end{figure*}

\subsection{Application Workload}
\label{subsec:app}

We first show the results of applications with potential data sharing in Rodinia benchmark
suite in Fig. \ref{fig:appspec}. For every benchmark, we use four different thread block sizes.
We show the original running time at different thread block sizes, denoted as {\em Original} in the
figure. We also show the running time
after applying our work partitioning techniques, denoted as {\em Optimized} in Fig.
\ref{fig:appspec}. The thread block size specifies how many threads can share data in
software-cache, since threads within the same block can see each other's data in software cache. 

\noindent {\bf B+tree} B+ tree is a tree data structure that keeps data sorted and allows
searches, sequential access, insertions, and deletions in logarithmic
time. It is commonly used in databases and file systems. A B+ tree can
be viewed as a B-tree in which each node contains only keys. The potential data sharing is the back and
forth movement over a path from root node to leaf node, which is handled by a set of threads in
parallel. The input is 10,000 queries into a database of 1 million records.

%The potential data reuse  By caching the data on the path in
%software cache, We improved the performance
%of {\em b+tree}'s findK kernel by 1.67 times and fingRangeK kernel by 1.41 times.

\noindent {\bf CFD} Computational fluid dynamics, usually abbreviated as CFD, is a branch
of fluid mechanics that uses numerical methods and algorithms to solve
and analyze problems that involve fluid flows. The fluid elements are simulated in an unstructured
grid. The potential data sharing occurs due to neighbour interactions  on the grid. The input is an
initial state of fluid with 97,046 fluid elements.

%The maximal degree in
%CFD data-affinity graph is 4. The order of the particles in memory or thread groups is typically determined
%by Hilbert space filling curve \cite{} since it is a good locality heuristic for dynamic scientific
%simulation code. We improved the performance of CFD upon the original partitioning obtained by
%Hilbert space filling curve by by over 18\%.

\noindent {\bf Gaussian} Gaussian Elimination computes results row by row, solving for variables in a
linear system. The algorithm synchronizes between iterations and the parallelism is exploited for value calculation in every
iteration. We focus on the kernel called {\em Fan2()} 
exhibits data sharing pattern within control flow statements. The input is a linear system with 1024
unknown variables.

%The data-affinity graph of Gaussian is
%very dense since it reuses data in cache significantly. However, the Gaussian application
%is also memory intensive, therefore we do not let data use hardware cache. With software cache
%(shared memory), the Gaussain performance is improved 2.19 times.

\noindent {\bf Particlefilter} The particle filter (PF) is statistical estimator of the location of
a target object given noisy measurements of that target's location and an idea of the object's path in a Bayesian framework. Particle filters or Sequential Monte Carlo (SMC) methods are a set of
on-line posterior density estimation algorithms. The potential data reuse happens when every
particle accesses the same density distribution function. The input is a tracking of 1,000
particles. 

%SMC methods use a grid-based approach,
%and use a set of particles to represent the posterior density. This kernel is computation
%intensive, and its global memory accesses is very small. As a result, although we reduce global memory transactions by 99.6\%, the performance
%improvement is only 4.8\%.

\noindent {\bf Streamcluster} Data Stream clustering, given a sequence of n points in a metric space and an integer k, output k points in the sequence to minimize the sum
of the distance of every point to its nearest neighborhood center. Data sharing occurs when every
thread tries to access the center points. The input is a set of 65536 data points with at maximum
1,000 centers.

%calculate distances of all points to a center point. Since all points are
%accessed for multiple times, we enhance cache sharing by modifying streamcluster to aggregate
%computation from every n iterations in 1 iteration, to explore sharing. Since aggregation
%has overhead, we set $n=2$. We use software cache and streamcluster performance is improved by
%19.9\%.




First, we can see from Fig. \ref{fig:appspec} that in most cases the optimized version performs better than the
original version when a thread block size is fixed. The maximum speedup is 2.2 times for {\em
particleFilter} at the thread block size 256. Every benchmark has significant speedup except {\em
streamcluster}. In {\em streamcluster}, the maximum speedup ~2\% is for thread block
size 1024. It is because streamcluster has less data sharing than other benchmarks at runtime. The
data that is reused is the center point. None of the other data points is reused, while the total number
of data points is 65535. Since only threads within a thread block can see each other's data, when
thread block size is smaller, the benefits are diminishing and there is no speedup, but also at
least no slowdown.   

Enlarging thread block size typically would enlarge the amount of sharing since more threads
share data, as illustrated in the {\em streamcluster} example. However, it is not always the case in the
our experiments. Depending on the workload data reuse pattern, when partitioning, it might cut more
nodes at the cluster boundary as the cluster size increases. And thus more data needs to be loaded
for a cluster. Recall that for our virtual cache design, we load all data objects of interest before
we carry out any computation a work cluster. In Fig. \ref{fig:appspec}, we find that CFD has best
performance of the optimized version for thread block size
320, among the thread block sizes of 192,256,320 and 384. 

It is noteworthy that even for the original program, different thread blocks imply performance
variation. The performance of GPU program depends on many execution parameters factors such as
occupancy, register usage per thread and original shared memory allocation. Regardless, not only our
transformed code usually performs better than the original at a fixed thread block size, but also
the best optimized version among all thread blocks performs better than the best original version
among all thread block sizes.    

\begin{figure}
\centering
\includegraphics[width=0.5\textwidth]{figures/summary.pdf}
\caption{Application performance summary}
\label{fig:appsummary}
\end{figure}

In Fig. \ref{fig:appsummary}, we show the comparison between the best optimized version and the best
original version across different thread block sizes, we still have significant performance gains or
at least no speedup for all benchmarks. In Fig. \ref{fig:appsummary}, we also show the comparison between the worst optimized version and
the worst original version, the baseline is the best original version. 


\subsection{Scale-free Workload}

The application workload in Section \ref{subsec:app} has the data sharing pattern of maximum reuse
frequency (maximum degree in locality graph) close to average reuse frequency (average degree in
locality graph), for instance, in CFD, the maximum number of neighbours of a fluid element is
bound by 4 and average is ~3, or simple scale-free pattern, for instance, in {\em streamcluster}, only one center node has maximum degree of
65535 and all others have degree of 1. In the second part of our evaluation, we select a workload
that exhibits {\em scale-free} locality graph pattern. That is, the degree distribution of the
locality graph, follows a power-law distribution. In another word, a set of nodes have large reuse
while the rest of nodes have few reuse.


\begin{table}[t]
\centering
\footnotesize
\caption{Matrices. Nnz: number of nonzero elments. AvgR: average reuse of a vector element.  MaxR:
maximum reuse of a vector element. }
%\scriptsize
%\begin{tabularx}{0.85\linewidth}{Xcccccc}
\begin{tabular}{|l|l|l|l|l|} \hline
Matrix & Nnz & Size & AvgR & MaxR\\
\hline
citationCiteseer & 2.3M & 268K$\times$268K & 5.50 & 1078   \\
IMDB  &  3.7M & 428K$\times$896K & 6.30 & 1590\\
web-Google  & 5.1M & 916K$\times$916K & 7.02  & 6326\\
web-NotreDame  & 1.4M & 325K$\times$325K & 6.45 & 10721\\
web-Stanford  & 2.3M & 281K$\times$281K & 8.51 & 38606 \\
wiki-Talk  &  5.0M & 2.4M$\times$2.4M & 3.99 & 100022\\
\hline
\end{tabular}
\label{tbl:spm}
\end{table}

We use the {\em spmv} kernel in \cite{CUSP} as baseline and use a set of sparse matrices with scale-free pattern
\cite{Tang+:CGO15}. We show the data reuse distribution of one of the six matrices in Fig.
\ref{fig:degdistribution} as they have similar pattern. We use {\em citatioCiteseer} as this
example. We use complement cumulative density function (CCDF) to represent the degree
distribution. A point (x,y) in CCDF figure represents that $y$ is the percentage of nodes that have
degree $>= x$. A graph that exhibits scale-free feature would see fast decaying of the CCDF
function. We also show the logarithmic scale of CCDF of {\em citationCiteseer} in
Fig. \ref{fig:degdistribution}.  We also show the statistics for these six matrices in Table
\ref{tbl:spm}.

\begin{figure}
\centering
\includegraphics[width=0.4\textwidth]{figures/spmv.pdf}
\caption{SPMV results for scale-free matrices}
\label{fig:spmv}
\end{figure}

We perform data-sharing aware work partitioning and show the results in Fig.
\ref{fig:spmv}. Unlike in Section \ref{subsec:app} we only report the performance of the kernel run without partition overhead.
For two reasons, first we transform the input sparse matrix file format so that the non-zero elements are
ordered in an order as if they would be executed by continuous logical threads. So we do not see
overhead when running the kernel. Secondly we only get the time of one kernel run (avg of many
repeated runs), while in practice, when the kernel is
called in a real application, it might run thousands of or millions of times, and thus the overhead of partitioning can be well
amortized. For the application workload in Section \ref{subsec:app}, the runtime partition overhead is
well amortized. If a kernel is run for only one time in an application, we do not suggest using the
work partitioning algorithm we presented in this paper. We will leave it as our future work
to further approximate the runtime partitioning algorithm. 

In Fig. \ref{fig:spmv}, we show the performance improvement over the kernel implemented in
CUSP \cite{CUSP} library. The performance enhancement can be seen as a potential to improve
performance for these sparse matrices as we do not take overhead into consideration. We have speed
up between 1.05 and 1.94. The matrix {\em wiki-talk} has a large maximum reuse, which is 100022
(Table \ref{tbl:spm}),
which means one of the input vector or output vector elements is reused significantly. However, the
average reuse is small which is 3.99, indicating a strong scale-free pattern. Our technique shows
significant improvement for the case, so is that for {\em web-Stanford}. For other cases, the
speedup is not significant, but no slow either. The baseline we compared to, the CUSP\cite{CUSP}
implementation, pre-process the data so that non-zero elements are sorted by their row number, it is
possible that the best partition is close to the one sorted by row index. Overall, based on results, for locality graph with strong
scale-free pattern, $deg_{max} >> deg_{avg}$, our technique show advantage. 







==> practical.tex <==

\iffalse

\begin{figure}
\centering
\includegraphics[width=0.5\textwidth]{figures/multiedge.pdf}
\caption{Preferentially grouped edges.}
\label{fig:pregroup}
\end{figure}

\subsection{Model Extension}

In realistic scenarios, there are data-affinity graphs with different features.
Using our basic EP model could not always achieve the best efficiency for all kinds of graphs.
Therefore, we extend our basic model to deal with certain types of data-affinity graphs.
Note that these extensions are not essential to the EP model.
%We show how to extend the basic model to handle complicated scenarios and how to efficiently control overhead.

\paragraph{Preferential grouping}

In practice, a computation task may consist of more than two operations (edges),
assuming one operation is a unit computation that uses two data operands. This is
usually specified by the programmer, who will specify which operations (edges)
should be preferred to be grouped together. These agglomerate operations should
not be split during workload partition. We handle this problem with
\emph{preferential grouping} in which we coarsen the graph by merging original edges
that should belong to the same group.

In \emph{preferential grouping}, we still perform a clone-and-connect
transformation in order to have a
vertex partition problem. However, we make slight adaptation in the
clone-and-connect stage. In the cloning stage, we only clone the vertices that
appear in different preferential groups of edges. In the connecting stage, we
connect cloned vertices with auxiliary edges to form a path for every set of
cloned vertices. Then we merge all original edges in every preferential group into a vertex.

We show an example of preferential grouping in Figure \ref{fig:pregroup}. Figure \ref{fig:pregroup} (a) shows the
original data-affinity graph. Figure \ref{fig:pregroup} (b) show there are
four preferential groups and show the graph after vertex cloning.  Figure
\ref{fig:pregroup} (c) shows the cloned vertices are connected, but this time, the
number of auxiliary edges added for every set of cloned vertices, corresponds to
the total number of preferential groups the cloned vertices fall into subtracted by
1. In Figure \ref{fig:pregroup} (d), we identify the preferential groups and
merge each group into one vertex. Figure \ref{fig:pregroup} (e) shows the
coarsened graph after edge merging.

The effect of preferential grouping is to make sure the edges that are specified
to be in the same group does not get assigned to different partitions. The
analytical bound still holds with slight modification on the $d_{max}-1$ factor.
Previously, the maximum degree $d_{max}$ is used to represent the worst case
scenario. Here, we use $g_{max}-1$ as the worst case approximation factor, where
$g_{max}$ is the maximum number of preferential edge groups a vertex falls into.
The proof is similar to the proof for Theorem \ref{thrm:bound}.

This preferential grouping technique also applies when one computation task
involves more than two data objects and we do not specify how the binary
operations are among these data objects. We still perform the above modified
clone-and-connect process followed by a merging of vertices in the same preferential
task group. The above bound holds as well.

%\begin{figure}[h]
%\centering
%%\includegraphics[width=0.4\textwidth]{figures/transactionload.pdf}
%\includegraphics[width=0.5\textwidth]{figures/citationCiteseer.pdf}
%\caption{CCDF of degree distribution for citationCiteseer}
%\label{fig:degdistribution}
%\end{figure}


\paragraph{Handling frequently reused data objects}

When one vertex in the data-affinity graph has a large degree such that its
incident edges consist of a large portion of the total number edges, for
instance $>50\%$, we can take advantage of this feature and use it to reduce
partition overhead. An example of such case is shown in Figure
\ref{fig:scalefree}. 8 out of the 9 vertices in the Figure \ref{fig:scalefree}(a) has
degree of 1 or 2 except one, which has degree of 7, and this vertex's 7 incident
edges comprise over 70\% of the total edges.

To reduce the partition overhead and maintain good partition results, we split
large-degree vertices first before the actual edge partition. We
define \emph{splitting} here as the process of duplicating a vertex the same number of times as its
degree and we do not add any auxiliary edge to the duplicated vertices. An example is
shown in Figure \ref{fig:scalefree} (b). Since a large-degree vertex's incident edges
constitute a significant portion of the total number of edges, assuming it is
$x\%$, then this vertex at least appears in x\% of the final work partitions by
pigeon hole rule. By
partitioning the split graph, in the worst case, a large-degree
vertex will appear in every work (edge) partition, but since it already has to
appear in a large percentage of clusters, the additional cost is small, which
is at most $100/x$ times the optimum.

Furthermore, we can reduce the worst case $100/x$
factor by placing this set of large-degree data objects into physical cache
(partitions) at once. Recall that in GPU execution model, one thread block can
be mapped to one SM only, but one SM can be mapped to multiple thread blocks,
which take turns to use cache (partitions), as if the cache is virtualized.
Since this set of data is shared by most of the thread blocks, we can load them
into physical cache once, and no matter how many thread blocks there are, we do
not have to reload this set of data whenever a thread block is scheduled. To
achieve this, we do not use software cache (shared memory), since in current programming model,
software cache (shared memory) is divided exclusively among thread blocks and different thread
blocks cannot share software cache (shared memory) data. We use hardware cache instead and we use texture cache or constant cache. These
cases may not happen often, but still exist in a type of important graphs
called scale-free graphs, in which the probability of the vertex degree follows a
power-law distribution. By splitting the graph first, we can reduce
the overhead of the ensuing edge partition since no auxiliary edges need to be
added for the set of duplicated large degree vertices. Figure
\ref{fig:scalefree} (b) and (c) show an example of 3-way edge partition on split
graphs.

\begin{figure}[h]
\centering
\includegraphics[width=0.45\textwidth]{figures/scalefree.pdf}
\caption{Handling frequently reused data node}
\label{fig:scalefree}
\end{figure}

\fi

\section{Applicability}
\label{sec:appl}

In this section, we will introduce how to apply our EP model to optimize data sharing for real GPU programs.
Figure \ref{fig:code_trans} shows an example of original and transformed code.
Software cache is used in this example to store shared data within thread blocks.

For the host function on CPU side (main() in Figure \ref{fig:code_trans}), first, it spawns another CPU thread to perform data sharing optimization.
The optimization process will be introduced in Section \ref{sect:appl:process}.
We use separate thread for optimization to prevent it from adversely affecting the performance of GPU kernel.
%In real programs, a kernel is usually executed multiple times.
Assume the GPU kernel is called multiple times.
Before every kernel call, we check if the optimization process has been completed.
If the answer is yes, the optimized kernel will be called with the optimized input.
Otherwise, the original kernel is called as usual.
The detail of our overhead control scheme as well as the situation when the GPU kernel is only called once will be discussed in Section \ref{sect:appl:overhead}.

For the kernel function on GPU side, there are three major modifications in order to leverage optimized input.
First, an array (local\_arrayA) is created in software cache to store shared data.
Then, each thread block loads its shared parts from the input array (opt\_arrayA) into the software cache array.
To avoid memory divergence which could cause severe performance degradation \cite{Zhang+:ASPLOS11, Wu+:PPoPP13}, adjacent threads are made to load adjacent data elements in the input array.
At last, we replace the reference of the original input array with that of the local array which resides in software cache.

\begin{figure}[htb]
	\centering
	\includegraphics[width=\linewidth]{figures/process.pdf}
	\caption{Example of code transformation.}
	\label{fig:code_trans}
\end{figure}

For the optimized kernel using texture cache, the host function needs to bind the optimized data layout to texture memory using the CUDA build-in function {\em cudaBindTexture()}.
The GPU kernel prefixes every data reference using function {\em tex1Dfetch()}. Then texture memory data are cached automatically by texture cache.

\subsection{Optimization Process}
\label{sect:appl:process}

Figure \ref{fig:workprocess} illustrates the working process of data sharing optimization.
The data access pattern of GPU programs are determined by both program semantics and input data.
Therefore, we extract data access pattern to build the data-affinity graph at first.

After data-affinity graph is built, we pre-examine the graph before actually partitioning it using EP model.
First, we check if there is enough data reuse by scanning the vertex degrees of data-affinity graph.
If there is no data reuse, or there is data reuse but the program's default scheduling is near optimal, we omit the partition process and use the original input.
%Alternatively, another possibility is we detect there is data reuse but the program's original schedule is near optimal.
%In this case, we omit the partition process and use the original schedule to produce the input of optimized kernel directly.
Second, we check if the graph fellows a special pattern such as clique, path, complete bipartite, and etc. during the graph building.
%First, we extract data access pattern according to program semantics and input and build the data-affinity graph.
For these special graphs, we can directly get the optimal task partition result without calling the EP model to reduce unnecessary partition overhead.

If we identify that task partition is necessary for the generated data-affinity graph, our EP model is applied on the graph to perform task partition as described in Section \ref{sec:tech}.

At last, we reorganize tasks among thread blocks based on the partition result by reordering input data layout.
In common GPU program model, a certain thread gets its task by reading a fixed location in the input data, and the location depends on the id of thread.
Therefore, we reorganize the data layout in the input (from arrayA to opt\_arrayA in Figure \ref{fig:code_trans}) to achieve the goal of rearranging tasks.
The mapping relationship from original to optimized data layout is also recorded and passed to the optimized kernel (opt\_indexA in Figure \ref{fig:code_trans}) to ensure correctness.
Besides, if shared data are loaded into software cache in the optimized kernel, we calculate the size of shared data within each thread block (beginA) to facilitate data loading of software cache.

\begin{figure}[htb]
	\centering
	\includegraphics[width=\linewidth]{figures/optimize_process.pdf}
	\caption{Optimization process.}
	\label{fig:workprocess}
\end{figure}

\subsection{Adaptive Overhead Control}
\label{sect:appl:overhead}

%Our adaptive overhead control consists of two components -- the static transformation component and dynamic adaptation component.

%\paragraph{Static transformation.}
%We perform source-to-source code transformation such that the transformed GPU kernel can take an task partition as input and execute correspondingly. To realize this, we replace every occurrence of a logical thread id in the kernel with a new logical thread id, for instance, in the irregular reference A[P[tid]] where tid denotes thread id, we transform it to A[P[tid']]. And at the beginning of a kernel, we insert a statement such that $ tid' = new\_task\_schedule[tid]$. This is similar to \emph{job swapping} transformation in \cite{Zhang+:ASPLOS11}. The \emph{new\_task\_schedule} is passed as an additional parameter to the kernel function and \emph{new\_task\_schedule} is obtained through runtime graph partitioning. We also transform the code to perform runtime data layout transformation if necessary (it is determined by dynamic adaptation component discussed below). We transform a memory reference A[P[tid]] to A'[P'[tid]] such that both A'[] and P'[] are obtained at runtime. In the static transformation components, we prepare multiple versions of the kernel, which would be dynamically selected at runtime.

%Furthermore, we also perform source-code analysis and check if special  graph patterns can be detected at compile-time including \emph{clique}, \emph{path}, \emph{complete bipartite graph} and etc. Since optimum edge partition can be achieved by taking advantage of these special graph patterns, we perform task partition statically and apply the \emph{new\_task\_schedule} via source-code transformation. This works for the programs that use linear array access indices, but not for the programs that use reference indirection. For these ones, we use dynamic adaptation discussed below.  

%\paragraph{Dynamic adaptation.}

To reduce overhead at runtime, we perform data sharing optimization using a separate thread on CPU while kernel is executed on GPU so that optimization process can run asynchronously.
We utilize a CPU-GPU pipelining technique to overlap computation and optimization for GPU programs \cite{Zhang+:ASPLOS11, Wu+:PPoPP13}.
%The approach of overlapping computation and optimization for GPU programs has been adopted in previous work \cite{Zhang+:ASPLOS11, Wu+:PPoPP13}.

In real GPU programs, a kernel is usually called multiple times, especially in scientific computation programs.
In such scenarios, We check if the asynchronous optimization is completed before calling the kernel and apply the optimization if so.
If the optimization work does not complete when the program finishes, we terminate it to guarantee no slowdown.
%A code example is shown in Figure \ref{fig:eff}.

%\begin{figure}[h]
%\centering
%\includegraphics[width=0.4\textwidth]{figures/efficiencyControl.pdf}
%\caption{Code example for efficiency control}
%\label{fig:eff}
%\end{figure}

If a kernel is only called once, we perform \emph{kernel splitting} \cite{Zhang+:ASPLOS11} which breaks one execution of a kernel into multiple executions of the same kernel with smaller number of threads.
Then we can apply the same method described above to amortize optimization overhead.
%Furthermore, if necessary, we perform data layout transformation. After graph partition, we check if spatial locality is deteriorated compared with original layout, and if so, we perform data layout transformation, we use \emph{cpack} algorithm described in \cite{Ding+:PLDI99} so that data objects within every task group are packed together as much as possible. If the partition and data layout transformation is completed before the end of the loop, we dynamically choose the right kernel to execute.

It is however possible that transformed kernel runs slower than the original kernel.
To prevent such cases from degrading performance of the overall execution, we record the transformed kernel time the first time it runs and compare it with the original kernel time.
If the first run of the transformed kernel is slower, we fall back to the original kernel in the next iteration.


